SceneGraphLoc: Cross-Modal Coarse Visual Localization on 3D Scene Graphs

We introduce a novel problem, i.e., the localization of an input image within a multi-modal reference map represented by a database of 3D scene graphs. These graphs comprise multiple modalities, including object-level point clouds, images, attributes, and relationships between objects, offering a lightweight and efficient alternative to conventional methods that rely on extensive image databases. Given the available modalities, the proposed method SceneGraphLoc learns a fixed-sized embedding for each node (i.e., representing an object instance) in the scene graph, enabling effective matching with the objects visible in the input query image. This strategy significantly outperforms other cross-modal methods, even without incorporating images into the map embeddings. When images are leveraged, SceneGraphLoc achieves performance close to that of state-of-the-art techniques depending on large image databases, while requiring three orders-of-magnitude less storage and operating orders-of-magnitude faster. The code will be made public.

==> tables/scan3r_val.tex <==
%\begin{table}[tb]
%  \caption{Recall of room retrieval task - Val Set in 3RScan. $R^t_{@*}$ means images are localized to re-scans of the same room. V3D means image to 3D place recognition; VPR means retrieval-based visual place recognition methods. }
%  \label{tab:headings}
%  \centering
%  \begin{tabular}{@{} | l | c c c | ccc | ccc | ccc | ccc@{}}
%  \multicolumn{1}{c|}{} &  \multicolumn{3}{c|}{Map modalities} &  \multicolumn{6}{c|}{10 rooms} & \multicolumn{6}{c}{All rooms} \\
%    \hline
%     Method & \phantom{--}$\mathcal{P}$\phantom{---} & \phantom{--}$\mathcal{I}$\phantom{--} & O & $R{@1}$ & $R{@3}$ & $R{@5}$ & $R^t_{@1}$ & $R^t_{@3}$ & $R^t_{@5}$ & $R{@1}$ & $R{@3}$ & $R{@5}$ & $R^t_{@1}$ & $R^t_{@3}$ & $R^t_{@5}$ \\
%    \hline
%     LidarCLIP~\cite{hess2024lidarclip} & \checkmark & \xmark & \xmark & 22.1 & 52.8 & 70.8 & 17.5 & 46.1 & 68.4 & 5.6 & 13.2 & 20.9 & 3.4 & 12.1 & 19.9\\
%     LIP-Loc~\cite{shubodh2024lip} & \checkmark & \xmark & \xmark & 29.9 & 53.7 & 69.6 & 24.0 & 55.4 & 71.8 & 7.2 & 24.8 & 35.8 & 7.1 & 27.7 & 39.0\\
%     % & Ours(GCVit) & 0.432 & 0.716 & 0.861 & 0.436 & 0.702 & 0.851  \\
%     OpenMask3D~\cite{takmaz2023openmask3d} & \checkmark & \xmark & \xmark & -- & -- & -- & 38.1 & 72.2 & 87.2 & -- & -- & -- & 16.2 & 35.9 & 50.0 \\
%    Proposed & \checkmark & \xmark & \checkmark & 62.3 & 87.7 & 96.5 & 62.0 & 87.4 & 96.5 & 49.6 & 66.1 & 75.6 & 49.2 & 65.8 & 75.4   \\
%     Proposed & \checkmark & \checkmark & \checkmark
%        & -- & -- & -- & 88.5 & 97.7 & 99.6  & -- & -- & -- & 80.6 & 91.6 & 95.2 \\
%    % & Ours (td-idf) & 0.586 & 0.853 & 0.953 & 0.586 & 0.858 & 0.958  \\
%     % & Ours w. 1 img/obj(GCVit) & -- & -- & -- & 0.637 & 0.858 & 0.944 \\
%     % & Ours w. 1 img/obj & -- & -- & -- & 0.825 & 0.971 & 0.992 \\
%    \hline
%     CVNet~\cite{lee2022correlation} & \xmark & \checkmark & \xmark& -- & -- & -- & 85.9 & 93.3 & 96.4 & -- & -- & -- & 80.7 & 87.3 & 90.1\\
%     AnyLoc~\cite{keetha2023anyloc} & \xmark & \checkmark & \xmark & -- & -- & -- & 93.6 & 98.0 & 99.4 & -- & -- & -- & 90.1 & 94.5 & 96.4  \\
%     %& CVNet w. 1 img/obj & -- & -- & -  & 80.3 & 90.8 & 95.4 \\
%     %& AnyLoc w. 1 img/obj  & -- & -- & -  & 89.3 & 97.5 & 99.4 \\
%    \hline
%  \end{tabular}
%\end{table}


% \begin{table}[tb]
%     \caption{Retrieval recall (\%; the target scene ranked within the top 1, 3, and 5 of the retrieved list) and storage requirements (MB) for methods utilizing point clouds ($\mathcal{P}$), images ($\mathcal{I}$), and other modalities (O) for map representation in the 3RScan dataset~\cite{3rscan}. Additionally, metrics for single-modal methods (CVNet and AnyLoc) reliant on extensive image datasets are presented. 
%     The results are reported for scenarios where the target room is chosen from a subset of 10 and the complete set of all (32) scenes.}
%   %Recall of room retrieval task - Val Set in 3RScan. $R^t_{@*}$ means images are localized to re-scans of the same room. V3D means image to 3D place recognition; VPR means retrieval-based visual place recognition methods. }
%   \label{tab:headings}
%   \centering
%   \resizebox{1.0\textwidth}{!}{\begin{tabular}{@{} | l | c c c | ccc | ccc | ccc | ccc | c |@{}}
%     \hline
%     \multicolumn{1}{|c|}{\multirow{2}{*}{Method}}
%      &  \multicolumn{3}{c|}{Map modalities} &  \multicolumn{6}{c|}{10 scenes} & \multicolumn{6}{c|}{All scenes} & Storage  \\
%       & \phantom{--}$\mathcal{P}$\phantom{---} & \phantom{--}$\mathcal{I}$\phantom{--} & O & $R{@1}$ & ${@3}$ & ${@5}$ & $R^t{@1}$ & ${@3}$ & ${@5}$ & $R{@1}$ & ${@3}$ & ${@5} $ & $R^t{@1}$ & ${@3}$ & ${@5}$ & (MB) \\
%     \hline
%      LidarCLIP~\cite{hess2024lidarclip} & \checkmark & \xmark & \xmark & 22.1 & 52.8 & 70.8 & 17.5 & 46.1 & 68.4 & \phantom{1}5.6 & 13.2 & 20.9 & \phantom{1}3.4 & 12.1 & 19.9 & \phantom{100}\textbf{0.38} \\
%      LIP-Loc~\cite{shubodh2024lip} & \checkmark & \xmark & \xmark & 29.9 & 53.7 & 69.6 & 24.0 & 55.4 & 71.8 & \phantom{1}7.2 & 24.8 & 35.8 & \phantom{1}7.1 & 27.7 & 39.0 & \phantom{100}1.01 \\
%      OMask3D~\cite{takmaz2023openmask3d} & \checkmark & \checkmark & \xmark & -- & -- & -- & 38.1 & 72.2 & 87.2 & -- & -- & -- & 16.2 & 35.9 & 50.0 & \phantom{10}20.13 \\
%     Proposed & \checkmark & \xmark & \checkmark & \textbf{62.3} & \textbf{87.7} & \textbf{96.5} & 62.0 & 87.4 & 96.5 & \textbf{49.6} & \textbf{66.1} & \textbf{75.6} & 49.2 & 65.8 & 75.4 & \phantom{100}5.35  \\
%      Proposed & \checkmark & \checkmark & \checkmark
%         & -- & -- & -- & \textbf{88.5} & \textbf{97.7} & \textbf{99.6}  & -- & -- & -- & \textbf{80.6} & \textbf{91.6} & \textbf{95.2} & \phantom{100}5.35 \\
%     \hline
%      CVNet~\cite{lee2022correlation} & \xmark & \checkmark & \xmark& -- & -- & -- & 85.9 & 93.3 & 96.4 & -- & -- & -- & 80.7 & 87.3 & 90.1 & \phantom{1}239.05 \\
%      AnyLoc~\cite{keetha2023anyloc} & \xmark & \checkmark & \xmark & -- & -- & -- & 93.6 & 98.0 & 99.4 & -- & -- & -- & 90.1 & 94.5 & 96.4 & 5720.29 \\
%     \hline
%   \end{tabular}}
% \end{table}


\begin{table}[tb]
    \caption{Retrieval recall (\%; the target scene ranked within the top 1, 3, and 5 of the retrieved list) and storage requirements (MB) for methods utilizing point clouds ($\mathcal{P}$), images ($\mathcal{I}$), and other modalities (O) for map representation in the 3RScan dataset~\cite{3rscan}. Additionally, metrics for single-modal methods (CVNet and AnyLoc) reliant on extensive image datasets are presented. 
    The results are reported for scenarios where the target room is chosen from a subset of 10 and the complete set of all (33) scenes.}
  %Recall of room retrieval task - Val Set in 3RScan. $R^t_{@*}$ means images are localized to re-scans of the same room. V3D means image to 3D place recognition; VPR means retrieval-based visual place recognition methods. }
  \label{tab:3drscan_results}
  \centering
  \resizebox{1.0\textwidth}{!}{\begin{tabular}{@{} | l | c c c | ccc | ccc | ccc | ccc | c |@{}}
    \hline
    \multicolumn{1}{|c|}{\multirow{2}{*}{Method}}
     &  \multicolumn{3}{c|}{Map modalities} &  \multicolumn{6}{c|}{10 scenes} & \multicolumn{6}{c|}{All scenes} & Storage  \\
      & \phantom{--}$\mathcal{P}$\phantom{---} & \phantom{--}$\mathcal{I}$\phantom{--} & O & $R{@1}$ & ${@3}$ & ${@5}$ & $R^t{@1}$ & ${@3}$ & ${@5}$ & $R{@1}$ & ${@3}$ & ${@5} $ & $R^t{@1}$ & ${@3}$ & ${@5}$ & (MB) \\
    \hline
     LidarCLIP~\cite{hess2024lidarclip} & \checkmark & \xmark & \xmark 
        & 22.1 & 52.8 & 70.8 & 17.5 & 46.1 & 68.4 & \phantom{1}5.6 & 13.2 & 20.9 & \phantom{1}3.4 & 12.1 & 19.9 & \phantom{100}\textbf{0.1} \\
     LIP-Loc~\cite{shubodh2024lip} & \checkmark & \xmark & \xmark 
        & 29.9 & 53.7 & 69.6 & 24.0 & 55.4 & 71.8 & \phantom{1}7.2 & 24.8 & 35.8 & \phantom{1}7.1 & 27.7 & 39.0 & \phantom{100}0.3 \\
     OMask3D~\cite{takmaz2023openmask3d} & \checkmark & \checkmark & \xmark 
        & -- & -- & -- & 38.1 & 72.2 & 87.2 & -- & -- & -- & 16.2 & 35.9 & 50.0 & \phantom{100}4.8 \\
    \textbf{SceneGraphLoc} & \checkmark & \xmark & \checkmark 
        & \textbf{62.3} & \textbf{87.7} & \textbf{96.5} & 62.0 & 87.4 & 96.5 & \textbf{49.6} & \textbf{66.1} & \textbf{75.6} & 49.2 & 65.8 & 75.4 & \phantom{100}1.5  \\
     \textbf{SceneGraphLoc} & \checkmark & \checkmark & \checkmark
        & -- & -- & -- & \textbf{88.5} & \textbf{97.7} & \textbf{99.6}  & -- & -- & -- & \textbf{80.6} & \textbf{91.6} & \textbf{95.2} & \phantom{100}1.5 \\
    \hline
     CVNet~\cite{lee2022correlation} & \xmark & \checkmark & \xmark
        & -- & -- & -- & 85.9 & 93.3 & 96.4 & -- & -- & -- & 80.7 & 87.3 & 90.1 & \phantom{10}64.3 \\
     AnyLoc~\cite{keetha2023anyloc} & \xmark & \checkmark & \xmark 
        & -- & -- & -- & 93.6 & 98.0 & 99.4 & -- & -- & -- & 90.1 & 94.5 & 96.4 & 1539.3 \\
    \hline
  \end{tabular}}
\end{table}



==> tables/scannet_val.tex <==
% \begin{table}[tb]
%   \caption{Recall of room retrieval task - Val Set of Predicted Scene Graph with SceneGraphFusion in Scannet. }
%   \label{tab:headings}
%   \centering
%   \begin{tabular}{@{}l | l | ccc | ccc | ccc @{}}

%     \multicolumn{2}{c|}{} &  \multicolumn{3}{c|}{$N_{rooms}$: 10} & \multicolumn{3}{c|}{$N_{rooms}$: 50}& \multicolumn{3}{c}{$N_{rooms}$: 98}\\
%     \hline
%      & Method & $R^t_{@1}$ & $R^t_{@3}$ & $R^t_{@5}$ & $R^t_{@1}$ & $R^t_{@3}$ & $R^t_{@5}$ & $R^t_{@1}$ & $R^t_{@3}$ & $R^t_{@5}$\\
%     \hline
%      \multirow{2}{*}{\rotatebox[origin=c]{90}{V3D}} 
%      & LidarCLIP & 22.1 & 52.8 & 70.8 & 3.4 & 12.1 & 19.9 & 1.6 & 6.0 & 11.3 \\
%      & LIP-Loc    & 13.7 & 32.8 & 41.4 & 8.8 & 12.3 & 13.1 & 3.1 & 6.9 & 11.3\\
%      % & Ours(GCVit) & 0.432 & 0.716 & 0.861 & 0.436 & 0.702 & 0.851  \\
%     & Ours, $\phi^{\{\mathcal{P, R, S}\}}$  & 54.5 & 84.1 & 94.9 & 31.0 & 50.6 & 61.9 & 23.4 & 39.9 & 49.3 \\
%     \hline
%      \multirow{3}{*}{\rotatebox[origin=c]{90}{VPR}} 
%      & OpenMask3D & 54.6 & 83.9 & 93.7 & 30.4 & 50.5 & 62.9 & 25.3 & 38.4 & 48.5 \\
%      & Ours, $\phi^{\{\mathcal{P, R, S, V}\}}$ 
%         & 83.1 & 95.8 & 99.2 & 66.7 & 82.9 & 94.0 & 57.1 & 78.4 & 90.0 \\
%      & CVNet & 96.3 & 98.5 & 99.3 & 92.4 & 96.5 & 97.4 & 90.3 & 94.9 & 96.1 \\
%      & AnyLoc & 98.7 & 99.6 & 99.8 & 97.5 & 98.6 & 99.1 & 97.0 & 98.5 & 98.9 \\
%     \hline
%   \end{tabular}
% \end{table}

\begin{table}[tb]
    \caption{Recall of room retrieval task - Val Set of Predicted Scene Graph with SceneGraphFusion in Scannet.
    The results are reported for scenarios where the target room is chosen from a subset of 10, 50 and the complete set of all (98) scenes.}
  %Recall of room retrieval task - Val Set in 3RScan. $R^t_{@*}$ means images are localized to re-scans of the same room. V3D means image to 3D place recognition; VPR means retrieval-based visual place recognition methods. }
  \label{tab:scannet_val_experi}
  \centering
  \resizebox{1.0\textwidth}{!}{\begin{tabular}{@{} | l | c c c | ccc | ccc | ccc | c |@{}}
    \hline
    \multicolumn{1}{|c|}{\multirow{2}{*}{Method}}
     &  \multicolumn{3}{c|}{Map modalities} &  \multicolumn{3}{c|}{10 scenes} & \multicolumn{3}{c|}{50 scenes} & \multicolumn{3}{c|}{All scenes} & Storage  \\
      & \phantom{--}$\mathcal{P}$\phantom{---} & \phantom{--}$\mathcal{I}$\phantom{--} & O & $R^t{@1}$ & ${@3}$ & ${@5}$ & $R^t{@1}$ & ${@3}$ & ${@5}$ & $R^t{@1}$ & ${@3}$ & ${@5}$ & (MB) \\
    \hline
     LidarCLIP~\cite{hess2024lidarclip} & \checkmark & \xmark & \xmark 
        & 22.1 & 52.8 & 70.8 & \phantom{1}3.4 & 12.1 & 19.9 & \phantom{1}1.6 & \phantom{1}6.0 & 11.3 & \phantom{100}\textbf{0.3} \\
     LIP-Loc~\cite{shubodh2024lip} & \checkmark & \xmark & \xmark 
        & 13.7 & 32.8 & 41.4 & \phantom{1}8.8 & 12.3 & 13.1 & \phantom{1}3.1 & \phantom{1}6.9 & 11.3 & \phantom{100}0.8\\
     OMask3D~\cite{takmaz2023openmask3d} & \checkmark & \checkmark & \xmark 
        & 54.6 & 83.9 & 93.7 & 30.4 & 50.5 & 62.9 & 25.3 & 38.4 & 48.5 & \phantom{100}9.5 \\
    Proposed & \checkmark & \xmark & \checkmark 
        & 54.5 & 84.1 & 94.9 & 31.0 & 50.6 & 61.9 & 23.4 & 39.9 & 49.3 & \phantom{100}5.0 \\
     Proposed & \checkmark & \checkmark & \checkmark
        & \textbf{83.1} & \textbf{95.8} & \textbf{99.2} & \textbf{66.7} & \textbf{82.9} & \textbf{94.0} & \textbf{57.1} & \textbf{78.4} & \textbf{90.0} & \phantom{100}5.0 \\
    \hline
     CVNet~\cite{lee2022correlation} & \xmark & \checkmark & \xmark
        & 96.3 & 98.5 & 99.3 & 92.4 & 96.5 & 97.4 & 90.3 & 94.9 & 96.1 & \phantom{10}53.8 \\
     AnyLoc~\cite{keetha2023anyloc} & \xmark & \checkmark & \xmark 
        & 98.7 & 99.6 & 99.8 & 97.5 & 98.6 & 99.1 & 97.0 & 98.5 & 98.9 & 1292.3 \\
    \hline
  \end{tabular}}
\end{table}

==> tables/tables_archive.tex <==
%\begin{table}[tb]
%  \caption{
%  Runtime and Memory on 3RScan Dataset: Val Set with 34 scans and 8197 images in Database and Test Set with 123 Scans and 30462 images in Database. 
%  $t_{2D}$ is the per-image time expense of the query image encoding, in milliseconds ($ms$); 
%  $t^N_{retrie}$ is the per-image time expense of coarse localization given $N$ candidate scenes ($N = 10,32$ for validation set and $N = 10,50$ for test set), in milliseconds ($ms$), 
%  and $S_{m}$ is the memory cost of the database of 3RScan validation set, in megabytes ($MB$).}
%  \label{tab:headings}
%  \centering
%  \begin{tabular}{@{}l | l | cccc | cccc @{}}
%  \multicolumn{2}{c|}{} & \multicolumn{4}{c|}{Val Set} & \multicolumn{4}{c}{Test Set} \\
%    \hline
%     & Method & $t_{2D}$ & $t^{10}_{retrie}$ & $t^{32}_{retrie}$ & $S_{m}$ 
%              & $t_{2D}$ & $t^{10}_{retrie}$ & $t^{50}_{retrie}$ & $S_{m}$ \\
%    \hline
%     \multirow{3}{*}{\rotatebox[origin=c]{90}{V3D}} 
%     & LidarCLIP & 4.2 & 0.15 & 0.22 & 0.10 & 4.1 & 0.14 & 0.29 & 0.38\\
%     & LipLoc & 2.7  & 0.07 & 0.12 & 0.28 &  2.7 & 0.07 & 0.18 & 1.01 \\
%     & Ours & 27.2 & 0.28 & 1.1 & 1.51 & 28.0 & 0.28 & 1.5 & 5.35 \\ 
%    \hline
%    \multirow{3}{*}{\rotatebox[origin=c]{90}{VPR}} 
%     & OpenMask3D & 55.9 & 0.49 & 5.81 & 4.75 & 41.5 & 4.78 & 7.40 & 20.13 \\
%     & CVNet & 14.1 & 7.05 & 30.8 & 64.32 & 14.3 & 9.00 & 60.01 & 239.05\\
%     & AnyLoc & 662.9 & 321.8 & 1901.81 & 1539.27 & 658.4 & 354.64 & 1826.39 & 5720.29\\
%    \hline
%  \end{tabular}
%\end{table}

%\begin{table}[tb]
%  \caption{
%  Runtime and Memory on Scannet Dataset: Val Set with 100 scans and 6892 images in Database and Test Set with 212 Scans and 14845 images in Database.}
%  \label{tab:headings}
%  \centering
%  \begin{tabular}{@{}l | l | cccc | ccccc @{}}
%  \multicolumn{2}{c|}{} & \multicolumn{4}{c|}{Val Set} & \multicolumn{5}{c}{Test Set} \\
%    \hline
%     & Method & $t_{2D}$ & $t^{10}_{retrie}$ & $t^{32}_{retrie}$ & $S_{m}$ 
%              & $t_{2D}$ & $t^{10}_{retrie}$ & $t^{50}_{retrie}$ & $t^{210}_{retrie}$  & $S_{m}$ \\
%    \hline
%     \multirow{3}{*}{\rotatebox[origin=c]{90}{V3D}} 
%     & LidarCLIP & 4.80 & 0.09 & 0.19 & 0.31  & 4.92 & 0.09 & 0.20& 0.62 & 0.65\\
%     & LipLoc & 3.64 & 0.12 & 0.23 & 0.82 & 4.09 & 0.12& 0.23& 0.52 & 1.72 \\
%     & Ours  & 22.9 & 1.33& 4.01& 4.95   & 16.60 & 1.32& 3.69 & 17.03& 9.30 \\ 
%    \hline
%    \multirow{3}{*}{\rotatebox[origin=c]{90}{VPR}} 
%     & OpenMask3D & 57.21 & 1.33 & 8.43 & 9.47  & 55.39 & 1.13 & 4.54 & 17.90 & 17.82 \\
%     & CVNet & 72.87 & 11.04 & 60.77& 53.84   & 53.98 & 10.58& 74.11& 311.26 & 115.98\\
%     & AnyLoc & 305.79 & 72.33 & 304.20 & 1292.25   & 242.99 & 68.22& 329.01& 1451.10& 2783.44\\
%    \hline
%  \end{tabular}
%\end{table}

% \begin{table}[tb]
%   \caption{Runtime and Memory - Test Set with 123 scans and 30462 images}
%   \label{tab:headings}
%   \centering
%   \begin{tabular}{@{}l | l | ccc @{}}
%     \hline
%      & Method & $T_{2D} (ms)$ & $T_{retrie} (ms)$ & $S_{map} (MB)$ \\
%     \hline
%      \multirow{2}{*}{\rotatebox[origin=c]{90}{V3D}} 
%      & LidarCLIP & 4.1 & 0.24 & 0.38 \\
%      & LipLoc    & 2.7 & 0.07 & 1.01 \\
%      \hline
%      & Ours & 28.0 & 0.28 & 5.35  \\
%     \hline
%      & OpenMask3D & 41.5 & 4.78 & 20.13 \\
%      \hline
%      \multirow{2}{*}{\rotatebox[origin=c]{90}{VPR}} 
%      & CVNet & 14.3 & 9.00 & 239.05 \\
%      & AnyLoc & 658.4 & 354.64 & 5720.29 \\
%     \hline
%   \end{tabular}
% \end{table}
